Challenges in the Design and Implementation of IoT Testbeds in Smart-Cities: A Systematic Review

Advancements in wireless communication and the increased accessibility to low-cost sensing and data processing IoT technologies have increased the research and development of urban monitoring systems. Most smart city research projects rely on deploying proprietary IoT testbeds for indoor and outdoor data collection. Such testbeds typically rely on a three-tier architecture composed of the Endpoint, the Edge, and the Cloud. Managing the system's operation whilst considering the security and privacy challenges that emerge, such as data privacy controls, network security, and security updates on the devices, is challenging. This work presents a systematic study of the challenges of developing, deploying and managing urban monitoring testbeds, as experienced in a series of urban monitoring research projects, followed by an analysis of the relevant literature. By identifying the challenges in the various projects and organising them under the V-model development lifecycle levels, we provide a reference guide for future projects. Understanding the challenges early on will facilitate current and future smart-cities IoT research projects to reduce implementation time and deliver secure and resilient testbeds.

==> Tables/author_projects.tex <==
\begin{table*}%[!h]
\makebox[1 \textwidth][c]{       %centering table
\resizebox{1 \textwidth}{!}{   


\begin{tabular}{llll}
\hline
\textbf{Project}                       & \textbf{Size (Where)}                                                                          & \textbf{Data collected}                                                                                  & \textbf{Architecture}             \\\hline
SPHERE                        & CS, (100 Homes), (1 EN; multiple EP)/home                                            & Environmental                                                & EN (802.15.4) $\rightarrow$ EN (4G) $\rightarrow$ CS           \\
UMBRELLA                      & CS, 200 EN (streetlamps) with on-board EP                                            & Environmental, Camera                                        & EP (I2C/SPI) $\rightarrow$ EN (Fibre/WiFi) $\rightarrow$ CS    \\
Cotham Hill Pedestrianization & CS, 10 EP in (8 homes)                                                               & Noise and air pollution                                      & EN (WiFi) $\rightarrow$ CS                                     \\
Residential Dampness          & (1 home), (1 EN with on-board EP)                                                    & Temperature, Humidity                                        & EP (Analog) $\rightarrow$ EN   \\
Clifton Suspension Bridge     & CS, 1 EN, X EP                                                                       & Structural health monitoring data                            & EP (802.15.4) $\rightarrow$ EN (4G) $\rightarrow$ CS           \\
Water quality monitoring      &                                                                                      & Water quality ()                                             &                                                                \\
SYNERGIA                      & CS, 3 ENs, 15 EP (office)                                                            & Environmental                                                & EP (802.15.4/LoRa) $\rightarrow$ EN (LAN) $\rightarrow$ CS     \\
REPLICATE (Energy)            & Smart appliances (151 Homes);                                                        & Energy consumption                                                                        &                                   \\
REPLICATE (eBike)             & CS, EN (12 e-bikes)                                                                  & battery level, motor power                                   & EP (CAN) $\rightarrow$ EN (LoRa/WiFi) $\rightarrow$ CS         \\
Bristol AoT                   & CS, 3 EN with on-board EP                                                            & Environmental, Camera                                        &  EP (I2C/SPI) $\rightarrow$ EN (4G) $\rightarrow$ CS           \\
Twinergy                          & 12 home                               & Energy consumption data                                       & EP (WiFi)          & $\rightarrow$ &                 & $\rightarrow$ & CS \\
EurValve                       & CS, (40 homes), (4 EN; 1 EP)/home                  & RSSI and accelerometer data                                                               & EP (Bluetooth) $\rightarrow$ EN (4G/WiFi)  $\rightarrow$ CS\\ \hline
\end{tabular}
} %close resize
}% %close centering
\caption{Research projects in which authors were involved. CS: Cloud Server, EN: Edge Node (Gateway), EP: Endpoints (IoT Node). CS may contain all or subset of open-source components (Kafka, K3S, MQTT, InfluxDB, Grafana). EN may consists of SBC (RPi or Intel NUC)}
\label{table:authors_involved}
\end{table*}

==> Tables/projects_referred.tex <==
\begin{table*}%[!h]
\makebox[1 \textwidth][c]{       %centering table
\resizebox{1 \textwidth}{!}{   


\begin{tabular}{llll}
\hline
\textbf{Project}                                   & \textbf{Size (Where)}                                                       & \textbf{Data collected}                                      & \textbf{Architecture}             \\\hline
AoT~\cite{Catlett2017}                             & CS, 130 EN (streetlamps) with on-board EP                                   & Environmental, Camera                                        & EP (I2C/SPI) $\rightarrow$ \hfill EN (4G) $\rightarrow$\hfill CS   \\
e-Agriculture~\cite{Oyedele2021}                   & EN (Lab deployment)                                                         & light, temperature, soil pH and humidity                     & EP (Analogue)$\rightarrow$EN               \\
Living Labs~\cite{Jackson2017}                     & CS, 150 EN, 800 EP (120 location)                                           & air quality, microclimating, bat monitoring                  & EP (RPL)$\rightarrow$EN (2G)$\rightarrow$CS \\
Connected Vehicle Testbed~\cite{Chowdhury2018}     & CS, 3 Fixed EN (FEN), 2 Mobile EN (MEN)                                     & Vehicle position data                                        & MEN (wireless)$\rightarrow$ FEN (wired)$\rightarrow$CS \\
Wireless Environmental Sensors~\cite{Folea2020}    & CS, 1 EN, 7 EP (Lab deployment)                                             & Environmental                                                & EP (Bluetooth)$\rightarrow$EN (LAN) $\rightarrow$ CS \\
Solar-powered WSN~\cite{Dehwah2015}                & 82 EP (real-world deployment)                                               & Temperature, RSSI, battery level                             & EP (WSN) w/ sink node \\
Community Elderly Care~\cite{Valera2018}           & CS, EN, EP (70 elderly homes)                                               & motion, door contact                                         & EP (Z-wave) $\rightarrow$ EN (cellular) $\rightarrow$ CS\\
IEEE802.15.4 Connectivity Traces~\cite{Traces2015} & 350 EP (Office environment)                                                 & RSSI, PDR                                                & EP (802.15.4) w/ sink node \\
LOFAR-Agro~\cite{Langendoen2006}                   & 109 EP, 3 EN, CS (real-world deployment)                                    & Temperature, humidity                                    & EP (WSN) w/ sink node $\rightarrow$ EN (WiFi)$\rightarrow$ CS \\
3E Houses~\cite{Porto2013}                         & CS, (100 homes)(6 EP/ 1 EN)/home                                            & Energy consumption data                                  & EP (Zigbee) $\rightarrow$ EN (WiFi) $\rightarrow$ CS \\
New York Noise sensor network~\cite{Mydlarz2019}   & CS, 55 Nodes (1 EP and 1 EN)/node                                           & Noise data                                               & EP (USB) $\rightarrow$ EN (WiFi) $\rightarrow$ CS \\
Padova Smart City~\cite{6918931}                   & CS, 1 EN, 8 EP                                                              & Temperature, humidity, benzene                           & EP (802.15.4) $\rightarrow$ EN (WiFi) $\rightarrow$ CS \\
Flash Flood Monitoring~\cite{Basnyat2020}          & 3 iter. of IoT device deployed; CS, EN, EP                                  & water levels                                             & EP (USB) $\rightarrow$ EN (cellular) $\rightarrow$ CS \\
Smart Santander~\cite{Sotres2017}                  & CS, 50+ EN, 700+ EP                                                         & environmental                                            & EP (802.15.4) $\rightarrow$ EN (Wired/Wireless) $\rightarrow$ CS \\
City of Things~\cite{Latre2016}                    & No details?                                                                 & air quality, traffic monitoring, parking                 & EP (WSN)$\rightarrow$ EN (multi-radio) $\rightarrow$ CS \\
SADMote~\cite{Elsts}                               & CS, 5 EN, 12 EP                                                             & Environmental                                            & EP (WSN) $\rightarrow$ EN (WiFi) $\rightarrow$ CS \\
SensorScope~\cite{Hnat2011}                        & CS, $\approx$6EN, each serving $\approx$100EP                               & Environmental                                            & EP (WSN) $\rightarrow$ EN (GPRS) $\rightarrow$ CS \\
EpiFi~\cite{Lundrigan2019}                         & $\approx$ 18 locations (2 EP, 1EN)/location                                 & Environmental                                            & EP (WSN/WiFI) $\rightarrow$ EN (WiFi) $\rightarrow$ CS \\
Parking System~\cite{Huang2017}                    & 2 EP, 3 EN                                                                  & Parking, Light sensor                                    & EP (Lora) $\rightarrow$ EN (Lora receiver/store on SD card)\\
Residential Sensing~\cite{Hnat2011}                & $\approx$ 20 homes $\approx$ 1200 EP                                        & Temperature, light, door                                 & EP (Z-wave) $\rightarrow$ EN (WiFi) $\rightarrow$ CS \\
Water consumption~\cite{Yang2015}                  & 30 homes, CS, 1EN, $\approx$ 4 EP                                           & Water consumption                                        & EP (433MHz) $\rightarrow$ EN (WiFi) $\rightarrow$ CS \\
\hline
\end{tabular}
} %close resize
}% %close centering
\caption{Research projects referred by the authors. Based on the details provided in the papers. CS: Cloud Server, EN: Edge Node, EP: Endpoints.}
\label{table:authors_referred}
\end{table*}


